Optimal Prediction using Learning and Shape Optimization

This paper investigates the problem of optimal predictor design for distributed parameter systems using neural networks and shape optimization. Sensors with various shapes are placed on the domain of the distributed parameter system. Data provided by these sensors are fed into a re-constructor to generate a full state of the system. After that, a trained neural-network predictor produces a prediction of the state at future time steps. The cost of prediction is defined as the weighted sensor area plus the squared norm of the prediction error. The location and shape of a sensor influences the prediction cost as well as the predictor performance. With the aid of the gradient of the network with respect to its inputs, an outer optimization layer is augmented to find optimized locations and shapes of the sensors. Simulation results show good agreement between the predicted and the true states as well as a significant reduction in cost by sensors with optimized locations and shapes.

==> numapde-bibliography/IntegrationTest/numapde-bibliography-dump-articles-main.tex <==
% Input the generated includes file
\IfFileExists{numapde-bibliography-dump-articles-includes.tex}{\input{numapde-bibliography-dump-articles-includes.tex}}{Run the \file{go.sh} script to generate the includes file.}

% Print the bibliography, by type
\section{@ARTICLE}
\numapdeprintbibliography[type=article,heading=none]



==> numapde-bibliography/IntegrationTest/numapde-bibliography-dump-nonarticles-main.tex <==
% Input the generated includes file
\IfFileExists{numapde-bibliography-dump-nonarticles-includes.tex}{\input{numapde-bibliography-dump-nonarticles-includes.tex}}{Run the \file{go.sh} script to generate the includes file.}

% Print the bibliography, by type
\section{@BOOK}
\numapdeprintbibliography[type=book,heading=none]

\section{@COLLECTION}
\numapdeprintbibliography[type=collection,heading=none]

\section{@INBOOK}
\numapdeprintbibliography[type=inbook,heading=none]

\section{@INCOLLECTION}
\numapdeprintbibliography[type=incollection,heading=none]

\section{@INPROCEEDINGS}
\numapdeprintbibliography[type=inproceedings,heading=none]

\section{@MANUAL}
\numapdeprintbibliography[type=manual,heading=none]

\section{@MISC}
\numapdeprintbibliography[type=misc,heading=none]

\section{@ONLINE}
\numapdeprintbibliography[type=online,heading=none]

\section{@PROCEEDINGS}
\numapdeprintbibliography[type=proceedings,heading=none]

\section{@REPORT}
\numapdeprintbibliography[type=report,heading=none]

\section{@THESIS}
\numapdeprintbibliography[type=thesis,heading=none]


==> numapde-latex/numapde-latex-documentation-main.tex <==
\tableofcontents

\section{Introduction}\label{sec:Introduction}

The idea of the material in our repository \url{\repositoryURL} is to provide a concise, reusable, and documented collection of \LaTeX\ commands, mainly for the purpose of creating manuscripts.
A typical beginning of the document preamble might look as simple as this:
\begin{lstlisting}[language={[LaTeX]TeX}]
\documentclass{numapde-preprint}
% Define often-used commands, load numapde-packages.sty, numapde-theorems.sty, numapde-syntax.sty
\usepackage{numapde-semantic}
% Configures style settings
\usepackage{numapde-style}
% Load optional packages if required
\usepackage{numapde-manifolds.sty}
% Define additional commands, override default settings
\usepackage{numapde-local}
\end{lstlisting}

The collection contains multiple parts:
\begin{itemize}
	\item
		a mechanism to load and configure often-used packages: \file{numapde-packages.sty} (\Cref{sec:packages}),
	\item
		their configuration, implementing a certain consistent style \file{numapde-style.sty} (\cref{sec:style}),
	\item
		the definition of colors \file{numapde-colors.sty} (\cref{sec:colors}),
	\item
		and individual commands, separated into
		\begin{itemize}
			\item
				syntactic \file{numapde-syntax.sty} (\Cref{sec:syntax})
			\item
				semantic \file{numapde-semantic.sty} (\Cref{sec:semantic}), further separated by topic for clarity
			\item
				local definitions \file{numapde-local.sty} (\Cref{sec:local-definitions}).
		\end{itemize}
\end{itemize}
This document provides a comprehensive overview of all packages and commands defined.
Packages are meant to used hierarchically, i.e, \file{numapde-manifolds.sty} builds upon and hence loads \file{numapde-semantic.sty}, which in turn builds upon and loads \file{numapde-packages.sty} and \file{numapde-syntax.sty}.
Additional commands and document specific settings should generally be defined locally initially in \file{numapde-local.sty} (\cref{sec:local-definitions}) and can make their way into the general collection later.

\textbf{Note 1.} Any changes to files in this repository need to be reflected in this file, \file{documentation.tex}, as well.

\textbf{Note 2.} If there are breaking changes, this package tries to provide old commands with warnings, if you load \file{numapde-deprecated.sty}.
While most old commands are loaded that way, commands that break with other packages,
symbols that break with other packages,
like \codeExample{\AA} or \codeExample{\SS} (which were used for calligraphic letters),
are not loaded in this legacy mode, neither.

\section{Packages: \texorpdfstring{\file{numapde-packages.sty}}{numapde-packages.sty}}\label{sec:packages}

The following packages are included by default, listed here in alphabetical order.\footnote{If you wish to add a package, please add it locally to your document via \file{numapde-local.sty}.}
% Last updated: 03.11.2020 from numapde-packages.sty

\begin{description}
	\item[academicons.sty] provides many academic icons (for \XeTeX{} processing only)
	\item[algpseudocode.sty*] provides environments and commands for typesetting of algorithms
	\item[amssymb.sty*] defines mathematical symbol fonts
	\item[amsthm.sty*] provides environments and styles, for example for typesetting proofs
	\item[babel.sty*] provides language dependent hyphenation patterns
	\item[biblatex.sty*] provides advanced bibliographic facilities, replaces \BibTeX%
	\item[booktabs.sty] enhances the quality of table typesetting
	\item[ccicons] to display creative commons license icons
	\item[changes.sty] allows to mark changes in documents
	\item[chngcntr.sty] allows to change the reset behavior for counters
	\item[cleveref.sty*] enhances cross referencing features
	\item[csquotes.sty] context sensitive quotation
	\item[enumitem.sty*] facilitates the customization of list type environments
	\item[fontenc.sty] enables the correct hyphenation of words with accents and umlauts
	\item[hyperref.sty*] enables hypertext referencing
	\item[ifthen.sty] facilitates the definition of conditional commands
	\item[ifxetex.sty] provides a way to check if a document is being processed by \XeTeX{} and company
	\item[inputenc.sty] supports in particular UTF8 inputs
	\item[listings.sty] provides source code formatting
	\item[longtable.sty] enables the typesetting of long tables
	\item[mathtools.sty] provides lots of improvements for math typesetting (includes \file{amsmath.sty})
	\item[moreenum.sty*] adds additional label styles to \file{enumitem.sty}
	\item[ntheorem.sty*] provides environments and styles, for example for typesetting proofs
	\item[siunitx.sty] facilitates the typesetting of numbers and SI units
	\item[stmaryrd.sty] defines a symbol font which includes, e.g., a double square bracket
	\item[xcolor.sty] extends \LaTeX's color facilities
	\item[xifthen.sty] extends \file{ifthen.sty} by adding new boolean conditions
	\item[xparse.sty] provides a high-level interface to define new commands
	\item[xspace.sty] adds space depending on context
\end{description}

An effort is made to achieve compatibility with many journals' \file{.cls} files.
Therefore, the packages marked with a star are not loaded when certain \file{.cls} files are in use.


\section{Syntax: \texorpdfstring{\file{numapde-syntax.sty}}{numapde-syntax.sty}}\label{sec:syntax}

The \file{numapde-syntax.sty} package provides mainly symbols and short commands, which can be used in semantic definitions for ease of notation.
They usually are rather simple commands without too many parameters.


\subsection{Letters}\label{subsec:letters}

\begin{commandlist}
	\item[ba\ldots bz] lower-case \textbf{b}old-face letters \mathCodeExample{\br, \bf}
	\item[bA\ldots bZ] upper-case \textbf{b}old-face letters \mathCodeExample{\bR, \bF}
	\item[balpha\ldots bomega] lower-case \textbf{b}old-face Greek letters \mathCodeExample{\balpha,\boldeta} (the latter being an exception)
	\item[bAlpha\ldots bOmega] upper-case \textbf{b}old-face Greek letters \mathCodeExample{\bGamma,\bDelta}
	\item[bnull] \textbf{b}old-face zero \mathCodeExample{\bnull}
	\item[bone] \textbf{b}old-face one \mathCodeExample{\bone}
	\item[cA\ldots cZ] upper-case \textbf{c}alligraphic letters \mathCodeExample{\cM, \cN}\\
	\numapdeWarning These symbols were called \codeCommand{\AA} etc.\ earlier. If your are migrating from a previous version you can use \codeCommand{\usepackage{numapde-deprecated}} to re-enable the old commands with a warning.
	\item[fA\ldots fZ] upper-case \textbf{f}raktur letters \mathCodeExample{\fM, \fN, \fX}\\
	\item[sA\ldots sZ] upper-case \textbf{s}cript letters \mathCodeExample{\sM, \sN, \sX}\\
	\item[va\ldots vz] lower-case letters with a \textbf{v}ector accent \mathCodeExample{\va,\vb}
	\item[vA\ldots vZ] upper-case letters with a \textbf{v}ector accent \mathCodeExample{\vA,\vB}
	\item[valpha\ldots vomega] lower-case Greek letters with a \textbf{v}ector accent \mathCodeExample{\valpha,\vbeta}
	\item[vAlpha\ldots vOmega] upper-case Greek letters with a \textbf{v}ector accent \mathCodeExample{\vGamma,\vDelta}
	\item[vnull] vector zero \mathCodeExample{\vnull}
	\item[vone] vector one \mathCodeExample{\vone}
	\item[C, K, N, Q, R, S, Z] mathematical sets \par\mathCodeExample{\C,\K,\N,\Q,\R,\S,\Z}
\end{commandlist}


\subsection{Phrases \& Names}\label{subsec:phrases_names}

It is useful to define commands for often-used phrases, abbreviations, and names in order to unify their notation.
All of the commands below are typeset using the command \codeCommand{\namemd}.
Its default definition is \codeCommand{\textsc{#1}\xspace}.\footnote{which adds a space if needed in textmode if needed, see \url{https://ctan.org/pkg/xspace} for details}
\begin{commandlist}
	\item[aa] almost all \codeExample{\aa}
	\item[adimat] \justCodeExample{\adimat}
	\item[ale] almost everwhere \codeExample{\ale}\\
	\numapdeWarning This was previously called \codeCommand{\ae} (which is reserved however for \justCodeExample{\ae}).
	\item[ampl] \justCodeExample{\ampl}
	\item[BibTeX] \justCodeExample{\BibTeX}
	\item[BibLaTeX] \justCodeExample{\BibLaTeX}
	\item[cg] \justCodeExample{\cg}
	\item[cpp] \justCodeExample{\cpp}
	\item[cppmat] \justCodeExample{\cppmat}
	\item[Dah] Das heißt (beginning of phrase) \codeExample{\Dah}
	\item[dah] das heißt \codeExample{\dah}
	\item[dolfin] \justCodeExample{\dolfin}
	\item[dolfinplot] \justCodeExample{\dolfinplot}
	\item[dolfinadjoint] \justCodeExample{\dolfinadjoint}
	\item[doxygen] \justCodeExample{\doxygen}
	\item[eg] exempli gratia (for example) \codeExample{\eg}
	\item[femorph] \justCodeExample{\femorph}
	\item[fenics] \justCodeExample{\fenics}
	\item[ffc] \justCodeExample{\ffc}
	\item[fmg] \justCodeExample{\fmg}
	\item[fortran] \justCodeExample{\fortran}
	\item[fs] fast sicher \codeExample{\fs}
	\item[fue] fast überall \codeExample{\fue}
	\item[gmres] \justCodeExample{\gmres}
	\item[gmsh] \justCodeExample{\gmsh}
	\item[IA] Im Allgemeinen (beginning of phrase) \codeExample{\IA}
	\item[iA] im Allgemeinen \codeExample{\iA}
	\item[idR] in der Regel \codeExample{\idR}
	\item[IdR] In der Regel (beginning of phrase) \codeExample{\IdR}
	\item[ie] id est (id est) \codeExample{\ie}
	\item[iid] independent and identically distributed \codeExample{\iid}
	\item[ipopt] \justCodeExample{\ipopt}
	\item[iW] im Wesentlichen \codeExample{\iW}
	\item[IW] Im Wesentlichen (beginning of phrase) \codeExample{\IW}
	\item[libsvm] \justCodeExample{\libsvm}
	\item[liblinear] \justCodeExample{\liblinear}
	\item[macmpec] \justCodeExample{\macmpec}
	\item[manifoldsjl] \justCodeExample{\manifoldsjl}
	\item[manopt] \justCodeExample{\manopt}
	\item[manoptjl] \justCodeExample{\manoptjl}
	\item[mathematica] \justCodeExample{\mathematica}
	\item[matlab] \justCodeExample{\matlab}
	\item[maple] \justCodeExample{\maple}
	\item[maxima] \justCodeExample{\maxima}
	\item[mE] meines Erachtens \codeExample{\mE}
	\item[metis] \justCodeExample{\metis}
	\item[minres] \justCodeExample{\minres}
	\item[mshr] \justCodeExample{\mshr}
	\item[mvirt] \justCodeExample{\mvirt}
	\item[numpy] \justCodeExample{\numpy}
	\item[oBdA] ohne Beschränkung der Allgemeinheit \codeExample{\oBdA}
	\item[OBdA] ohne Beschränkung der Allgemeinheit (beginning of phrase) \par\codeExample{\OBdA}
	\item[og] oben genannt \codeExample{\og}
	\item[oae] oder ähnliche \codeExample{\oae}
	\item[paraview] \justCodeExample{\paraview}
	\item[pdflatex] \justCodeExample{\pdflatex}
	\item[perl] \justCodeExample{\perl}
	\item[petsc] \justCodeExample{\petsc}
	\item[pymat] \justCodeExample{\pymat}
	\item[python] \justCodeExample{\python}
	\item[scikit] \justCodeExample{\scikit}
	\item[scikitlearn] \justCodeExample{\scikitlearn}
	\item[scipy] \justCodeExample{\scipy}
	\item[sphinx] \justCodeExample{\sphinx}
	\item[spd] symmetric positive definite \codeExample{\spd}
	\item[so] siehe oben \codeExample{\so}
	\item[st] such that or subject to \codeExample{\st}
	\item[subgmres] \justCodeExample{\subgmres}
	\item[subminres] \justCodeExample{\subminres}
	\item[superlu] \justCodeExample{\superlu}
	\item[svmlight] \justCodeExample{\svmlight}
	\item[tritetmesh] \justCodeExample{\tritetmesh}
	\item[ua] unter anderem \codeExample{\ua}
	\item[Ua] Unter anderem (beginning of phrase) \codeExample{\Ua}
	\item[ufl] \justCodeExample{\ufl}
	\item[ug] unten genannt \codeExample{\ug}
	\item[uqlab] \justCodeExample{\uqlab}
	\item[uU] unter Umständen \codeExample{\uU}
	\item[UnU] Unter Umständen (beginning of phrase) \codeExample{\UnU}
	\item[viper] \justCodeExample{\viper}
	\item[wrt] with respect to \codeExample{\wrt}
	\item[xml] \justCodeExample{\xml}
	\item[zB] zum Beisiel \codeExample{\zB}
	\item[ZB] Zum Beispiel (beginning of phrase) \codeExample{\zB}
	\item[zHd] zu Händen \codeExample{\zHd}
\end{commandlist}


\subsection{Syntax Helpers}\label{subsec:syntax_helpers}

\begin{commandlist}
	\item[enclspacing] provides spacing after the opening and before the closing delimiters for \codeCommand{\enclose}.
		This is by default set to be empty.
	\item[enclose] is a command which encloses some content in scaled delimiters.
		It is meant as a helper to facilitate the definition of other commands.
		Its syntax is \codeCommand{\enclose[#1]{#2}{#3}{#4}}.
		The first (optional) argument is used to scale the delimiters to the standard amsmath sizes.%
		\footnote{\lstinline!big!, \lstinline!Big!, \lstinline!bigg!, \lstinline!Bigg! or \lstinline!auto!, which uses \lstinline!left! and \lstinline!right! as well as \lstinline!none! to easily deactivate brackets.\label{footnote:amsmath_sizes}}
		The second and fourth arguments specify the opening and closing delimiters, respectively.
		The third argument is the content to be enclosed.
		\par\mathCodeExample{\enclose{[}{\dfrac{1}{2}}{]}} % chktex 9
		\par\mathCodeExample{\enclose[Big][{\dfrac{1}{2}}]} % chktex 9
		\par\mathCodeExample{\enclose[auto]{[}{\dfrac{1}{2}}{]}} % chktex 9
		\par\mathCodeExample{\enclose[none]{[}{\dfrac{1}{2}}{]}} % chktex 9

		\textbf{Note 1.} \lstinline!none! is merely meant for testing when having arguments
		in brackets whether it is useful to omit them. You can also deactivate the absolute value
		vertical lines this way, so \emph{use this option with care}.

		\textbf{Note 2.} This command should normally be used only in the definition of other commands.
		For instance, \codeCommand{\abs} is using it internally. See \codeCommand{\paren} for the nicer command to use
	\item[enclspacingSet] provides spacing before and after the center delimiter \codeCommand{\encloseSet}.
		This is by default set to \codeCommand{\,}.
	\item[encloseSet] is a command which encloses some content in scaled delimiters.
		It is meant as a helper to facilitate the definition of other commands.
		Its syntax is \codeCommand{\encloseSet#1]{#2}{#3}{#4}{#5}{#6}}.
		The first (optional) argument is used to scale the delimiters including the center one to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second and sixth arguments specify the opening and closing delimiters, respectively.
    The fourth argument specifies the center delimiter and
		The third and fifth argument are the content to be enclosed.
		\par\mathCodeExample{\encloseSet[big]{\{}{x\in\R}{|}{x>5}{\}}} % chktex 9
		\par\mathCodeExample{\encloseSet[auto]{\{}{x\in\R}{|}{x>\dfrac{1}{2}}{\}}} % chktex 9
		\\
		\textbf{Note.} This command should normally be used only in the definition of other commands.
		For instance, \codeCommand{\setDef} is using it internally.
	\item[paren] is an alternative to \codeCommand{\enclose}, with a different ordering of arguments.
		Its syntax is \codeCommand{\paren[#1]{#2}{#3}{#4}}, which is simply mapped to \codeCommand{\enclose[#1]{#2}{#4}{#3}}.
		\par\mathCodeExample{\paren[Big]{[}{]}{\dfrac{1}{2}}}
		\par\mathCodeExample{\paren[Big][]{\dfrac{1}{2}}}
		\par\mathCodeExample{\paren[auto]{[}{]}{\dfrac{1}{2}}}
\end{commandlist}


\subsection{Spacing Helpers}\label{subsec:spacing_helpers}

\begin{commandlist}
	\item[clap] complements the standard \LaTeX\ commands \codeCommand{\llap} and \codeCommand{\rlap}.
		These commands horizontally smash their arguments.
		\par\codeExample{Let us \llap{smash} something.}
		\par\codeExample{Let us \clap{smash} something.}
		\par\codeExample{Let us \rlap{smash} something.}
	\item[mathllap] corresponds to \codeCommand{\llap} in math mode.
		\par\mathCodeExample{\sum_{\mathllap{1\le i\le j\le n}} X_{ij}}
	\item[mathclap] corresponds to \codeCommand{\clap} in math mode.
		\par\mathCodeExample{\sum_{\mathclap{1\le i\le j\le n}} X_{ij}}
	\item[mathrlap] corresponds to \codeCommand{\rlap} in math mode.
		\par\mathCodeExample{\sum_{\mathrlap{1\le i\le j\le n}} X_{ij}}
	\item[mrep] stands for \emph{math replace} and it typesets an argument while reserving the space for another.
		Its syntax is \codeCommand{\mrep[#1]{#2}{#3}}
		The first (optional) argument is one of \codeCommand{{l,c,r}} and it is used to define the alignment.
		\codeCommand{c} is the default.
		\par\mathCodeExample{\mrep[l]{1}{-1}-1}
		\par\mathCodeExample{\mrep[c]{1}{-1}-1}
		\par\mathCodeExample{\mrep[r]{1}{-1}-1}
\end{commandlist}


\section{Semantic: \texorpdfstring{\file{numapde-semantic.sty}}{numapde-semantic.sty}}\label{sec:semantic}

Semantic commands provide commands that can be used in any
of the forthcoming topics and are of interest for all, but
are not on a symbol level but have a certain meaning.
This might even be only a convention, for example when defining
a notion for an inner product.
\begin{commandlist}
	\item[abs] absolute value.
		Its syntax is \codeCommand{\abs[#1]{#2}}.
		The first (optional) argument is used to scale the deliminters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		\par\mathCodeExample{\abs{a}}
		\par\mathCodeExample{\abs[Big]{\dfrac{1}{2}}}
		\par\mathCodeExample{\abs[auto]{\dfrac{1}{2}}}
	\item[aff] affine hull \mathCodeExample{\aff}
	\item[arcosh] area hyperbolic cosine \mathCodeExample{\arcosh}
	\item[arcoth] area hyperbolic cotangens \mathCodeExample{\arcoth}
	\item[argmax] maximizer of a function
		\mathCodeExample{\argmax_{x \in \R} f(x)} % chktex 6
	\item[Argmax] set of maximizers of a function
		\mathCodeExample{\Argmax_{x \in \R} f(x)} % chktex 6
	\item[argmin] minimizer of a function
		\mathCodeExample{\argmin_{x \in \R} f(x)} % chktex 6
	\item[Argmin] set of minimizers of a function
		\mathCodeExample{\Argmin_{x \in \R} f(x)} % chktex 6
	\item[arsinh] area hyperbolic cotangens \mathCodeExample{\arsinh}
	\item[artanh] area hyperbolic tangens \mathCodeExample{\artanh}
	\item[bdiv] bold (meaning: vector) divergence of a matrix-valued function \mathCodeExample{\bdiv}
	\item[ceil] integer larger or equal to input.
		Its syntax is \codeCommand{\ceil[#1]{#2}}.
		The first (optional) argument is used to scale the deliminters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		\par\mathCodeExample{\ceil{a}}
		\par\mathCodeExample{\ceil[Big]{\dfrac{1}{2}}}
	\item[clconv] closure of the convex hull of a set \mathCodeExample{\clconv M}
	\item[closure] closure of a set \mathCodeExample{\closure M}
	\item[cofac] cofactor matrix \mathCodeExample{\cofac(A)}
	\item[compactly] compact embedding of topological spaces \mathCodeExample{\compactly}
	\item[cone] conic hull \mathCodeExample{\cone}
	\item[conv] convex hull of a set \mathCodeExample{\conv M}
	\item[corresponds] binary operator for correspondence \mathCodeExample{A\corresponds B}
	\item[cov] covariance \mathCodeExample{\cov}
	\item[curl] the curl operator \mathCodeExample{\curl}
	\item[d] integral symbol with prepended space, as in
		\par\mathCodeExample{\int_\R \exp(-x^2) \d x}
	\item[dev] deviator of a matrix \mathCodeExample{\dev A}
	\item[diag] diagonal matrix composed of entries in a vector, or diagonal of a matrix
		\par\mathCodeExample{\diag(a)}
		\par\mathCodeExample{\diag(A)}
	\item[diam] diameter \mathCodeExample{\diam(M)}
	\item[distOp] the mathematical operator denoting the distance
		\par\mathCodeExample{\distOp}
	\item[dist] distance from a point to a set.
		Its syntax is \codeCommand{\dist[#1]{#2}{#3}} or \codeCommand{\dist[#1]{#2}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the point; it can be omitted.
		The command \codeCommand{\distOp} is used to typeset the operator.
		\par\mathCodeExample{\dist[Big]{\cC}{\dfrac{x}{2}}}
		\par\mathCodeExample{\dist{\cC}}
		\par\mathCodeExample{\dist}
	\item[div] divergence \mathCodeExample{\div}
	\item[Div] (row-wise) divergence \mathCodeExample{\Div}
	\item[dom] domain \mathCodeExample{\dom}
	\item[dotcup] distinct union \mathCodeExample{\dotcup}
	\item[dprod] double contraction of matrices $A \dprod B = \sum_{i,j} A_{ij} B_{ij} = \trace(A^\transp B)$
		\par\mathCodeExample{A \dprod B}
	\item[dual] duality pairing.
		Its syntax is \codeCommand{\dual[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the delimiters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the first factor.
		The third argument denotes the second factor.
		\par\mathCodeExample{\dual{x^*}{x}}
		\par\mathCodeExample{\dual[Big]{x^*}{\dfrac{1}{2}}}
	\item[e] Euler's number \mathCodeExample{\e}
	\item[embed] embedding of topological spaces \mathCodeExample{\embed}
	\item[embeds] synonym of \codeCommand{\embed} \mathCodeExample{\embeds}
	\item[epi] epigraph \mathCodeExample{\epi}
	\item[eR] extended real line \mathCodeExample{\eR = \R \cup \{\pm \infty\}}
	\item[essinf] essential infimum \par \mathCodeExample{\displaystyle\essinf_{x \in \R} f(x)} % chktex 1 chktex 6
	\item[esssup] essential supremum \par \mathCodeExample{\displaystyle\esssup_{x \in \R} f(x)} % chktex1 chktex 6
	\item[file] typesets a file name (using \codeCommand{nolinkurl})
		\par\codeExample{\file{test.txt}}
	\item[floor] integer less or equal to input.
		Its syntax is \codeCommand{\floor[#1]{#2}}.
		The first (optional) argument is used to scale the delimiters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		\par\mathCodeExample{\floor{a}}
		\par\mathCodeExample{\floor[Big]{\dfrac{1}{2}}}
	\item[grad] gradient (of a function) \mathCodeExample{\grad F} %chktex 1
	\item[Graph] graph of a function \mathCodeExample{\Graph}
	\item[id] identity operator \mathCodeExample{\id}
	\item[image] image of a function \mathCodeExample{\image}
	\item[inj] injedctivity (radius) \mathCodeExample{\inj}
	\item[inner] inner product.
		Its syntax is \codeCommand{\inner[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parentheses enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the first factor.
		The third argument denotes the second factor.
		\par\mathCodeExample{\inner{a}{b}}
		\par\mathCodeExample{\inner[Big]{a}{\dfrac{b}{2}}}
	\item[interior] \mathCodeExample{\interior}
	\item[jump] jump of a quantity, \eg, across a finite element facet.
		Its syntax is \codeCommand{\jump[#1]{#2}}.
		The first (optional) argument is used to scale the delimiters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		\par\mathCodeExample{\jump{a}}
		\par\mathCodeExample{\jump[Big]{\dfrac{1}{2}}}
	\item[laplace] the Laplace operator \mathCodeExample{\laplace u} %chktex 1
	\item[lin] linear hull of a set of vectors \mathCodeExample{\lin\{v_1,v_2\}}
	\item[norm] norm of a vector.
		Its syntax is \codeCommand{\norm[#1]{#2}}.
		The first (optional) argument is used to scale the delimiters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		\par\mathCodeExample{\norm{a}}
		\par\mathCodeExample{\norm[Big]{\dfrac{c}{2}}}
		\par\mathCodeExample{\norm[auto]{\dfrac{c}{2}}}
		%
	\item[projOp] the mathematical operator denoting the projection \mathCodeExample{\projOp}
		\par\mathCodeExample{\projOp}
	\item[proj] projection onto a set.
		Its syntax is \codeCommand{\proj[#1]{#2}(#3)} or \codeCommand{\proj[#1]{#2}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set and can also be left out.
		The third argument denotes the point; it can be omitted.
		The command \codeCommand{\projOp} is used to typeset the operator.
		\par\mathCodeExample{\proj}
		\par\mathCodeExample{\proj(x)}
		\par\mathCodeExample{\proj{\cC}}
		\par\mathCodeExample{\proj{\cC}(x)}
		\par\mathCodeExample{\proj[Big](\dfrac{x}{2})}
		\par\mathCodeExample{\proj[Big]{\cC}(\dfrac{x}{2})}
	\item[proxOp] the mathematical operator denoting the proximal map
		\par\mathCodeExample{\proxOp}
	\item[prox] the proximal operator of a function.
		Its syntax is \codeCommand{\prox[#1]{#2}(#3)} or \codeCommand{\prox[#1]{#2}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the point; it can be omitted.
		The command \codeCommand{\proxOp} is used to typeset the operator.
		\par\mathCodeExample{\prox}
		\par\mathCodeExample{\prox{\lambda F}} % chktex 1
		\par\mathCodeExample{\prox{\lambda F}(x)} % chktex 1
		\par\mathCodeExample{\prox[auto]{\lambda F}(\dfrac{x}{2})} %chktex 1
	\item[rank] rank (of a matrix) \mathCodeExample{\rank}
	\item[range] range of some operator \mathCodeExample{\range}
	\item[restr] restriction/evaluation.
		Its syntax is \codeCommand{\restr[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the deliminters enclosing the arguments to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument to be restricted/evaluated.
		The third argument denotes the restriction set/evaluation point.
		\par\mathCodeExample{\restr[auto]{\frac{\d}{\d t}(f \circ \gamma)(t)}{t=0}}
	\item[ri] relative inerior \mathCodeExample{\ri}
  \item[setDef] define a set, where \codeCommand{\setMid} serves as the center divider.
		Its syntax is \codeCommand{\setDef[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument and the center divider to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the left part of the definition, naming the potential elements of the set being defined.
		The third argument denotes the condition to include the elements in the set.
		\par\mathCodeExample{\setDef{x\in\R}{x>5}}\\
		\par\mathCodeExample{\setDef[Big]{x\in\R}{x>\dfrac{1}{2}}}
	\item[setMid] divider within \codeCommand{\setDef} (set definitions).
		This is by default set to \codeCommand{|}.
	\item[sgn] sign \mathCodeExample{\sgn}
	\item[Sgn] sign (set valued) \mathCodeExample{\Sgn}
	\item[supp] support (of a function) \mathCodeExample{\supp F} % chktex 1
	\item[sym] symmetric part (of a matrix) \mathCodeExample{\sym A} % chktex 1
	\item[trace] trace (of a matrix) \mathCodeExample{\trace A}  % chktex 1
	\item[transp] transpose of a vector or matrix.
		\par\mathCodeExample{A^\transp}
	\item[transposeSymbol] symbol to use for the transpose
		\par\mathCodeExample{\transposeSymbol}
	\item[var] variance \mathCodeExample{\var}
	\item[weakly] weak convergence of a sequence \mathCodeExample{\weakly}
	\item[weaklystar] weak star convergence of a sequence \mathCodeExample{\weaklystar}
\end{commandlist}


\section{Theorem-Like Environments: \texorpdfstring{\file{numapde-theorems.sty}}{numapde-theorems.sty}}\label{sec:theorems}

\file{numapde-theorems.sty} ensures that the following theorem-like environments are always available:
\begin{commandlist}
	\item \codeCommand{assumption}  and \codeCommand{assumption*}
	\item \codeCommand{corollary}   and \codeCommand{corollary*}
	\item \codeCommand{definition}  and \codeCommand{definition*}
	\item \codeCommand{example}     and \codeCommand{example*}
	\item \codeCommand{lemma}       and \codeCommand{lemma*}
	\item \codeCommand{proposition} and \codeCommand{proposition*}
	\item \codeCommand{remark}      and \codeCommand{remark*}
	\item \codeCommand{theorem}     and \codeCommand{theorem*}
\end{commandlist}
and a \codeCommand{proof} environment.
Depending on the \file{.cls} file of the main document loaded, different mechanisms are used to provide these environments.
Compatibility with \file{cleveref.sty} is ensured.
Whenever possible, theorem-like environments will share a counter.


\section{Additional Semantics by Topic}\label{sec:semantics-by-topic}

While semantic commands might be suitable for all mathematical topics, the following subsections collect commands which are most useful in one particular mathematical area and hence might clutter the general semantic file.
Any semantic topic files should always build on \file{numapde-semantic.sty}.


\subsection{Manifolds: \texorpdfstring{\file{numapde-manifolds.sty}}{numapde-manifolds.sty}}\label{subsec:manifolds}

The semantic file \file{numapde-manifolds.sty} collects definitions and notations for Riemannian manifolds.
\begin{commandlist}
	\item[bitangent] the bitangent space.
		Its syntax is \codeCommand{\bitangent{#1}[#2]}.
		The first argument denotes the base point.
		The second (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\bitangent{p}}
		\par\mathCodeExample{\bitangent{q}[\cN]}
	\item[bitangentSpaceSymbol] the symbol used within \codeCommand{\bitangent}.
		\par\mathCodeExample{\bitangentSpaceSymbol}
	\item[cotangent] the cotangent space.
		Its syntax is \codeCommand{\cotangent{#1}[#2]}.
		The first argument denotes the base point.
		The second (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\cotangent{p}}
		\par\mathCodeExample{\cotangent{q}[\cN]}
	\item[cotangentBundle] the cotangent bundle.
		Its syntax is \codeCommand{\cotangentBundle[#1]}.
		The (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\cotangentBundle}
		\par\mathCodeExample{\cotangentBundle[\cN]}
	\item[cotangentSpaceSymbol] the symbol used within \codeCommand{\cotangent}.
		\par\mathCodeExample{\cotangentSpaceSymbol}
	\item[covariantDerivative] is the covariant derivative.
		Its syntax is \codeCommand{\covariantDerivative{#1}[#2]}.
		The first argument is the vector (or vector field) determining the direction of differentiation.
		The second (optional) argument denotes the tensor field being differentiated.
		\par\mathCodeExample{\covariantDerivative{X}{Y}}
	\item[covariantDerivativeSymbol]\hspace{4em}the symbol used for the covariant derivative \codeCommand{\covariantDerivative}.
		\par\mathCodeExample{\covariantDerivativeSymbol}
	\item[exponential] the exponential map.
		Its syntax is \codeCommand{\exponential[#1]{#2}{#3}}.
		The first argument can be used to scale the third.
		The second argument denotes the base point and is optional.
		The third argument denotes the tangent vector, which is optional, but if provided, the argument is put in brackets.
		The first following example illustrates the case, where no brackets are put.
		Note that the space is mandatory.
		\par\mathCodeExample{\exponential{p}X}
		\par\mathCodeExample{\exponential{p}(X)}
		\par\mathCodeExample{\exponential[Big]{p}(\frac{X}{2})}
	\item[expOp] the symbol used within the \codeCommand{\exponential}.
		\par\mathCodeExample{\expOp}
	\item[geodesic] a geodesic.
		Its syntax is \codeCommand{\geodesic|#1|<#2>[#3]{#4}{#5}(#6)}.% chktex 6
		The first argument can be used to use a different symbol (locally) for the geodesic
		The second (optional) argument is used to modify the style of the geodesic (\codeCommand{s}ymbol, \codeCommand{l}ong, \codeCommand{a}rc or \codeCommand{p}lain, where the last is the default)
		The third (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		It is ignored when the sixth argument is not given.
		The fourth argument denotes the initial point (at $t = 0$).
		The fifth argument denotes either the final point (at $t = 1$) for types~\codeCommand{l} and \codeCommand{a}, or the initial tangent vector for type~\codeCommand{p}.
		The sixth (optional) argument denotes the evaluation point.
		The command \codeCommand{\geodesicSymbol} is used to typeset the geodesic symbol default (i.e. globally)
		% \begin{itemize}
		% 	\item a style might be given in \lstinline!<>! as first, optional argument
		% 	\item the second argument in \lstinline![]! is again scaling of the argument (ignored for \lstinline!s! or if the last is not given)
		% 	\item the third and fourth in usual curly braces are also optional and refer to either start and end point or start point and tangent,
		% 	\item the argument of the geodesic is given in \lstinline!()! as fifth argument
		% \end{itemize}
		% Note that omiting the third and fourth might lead to undesired print, especially for \lstinline!l!ong.
		\par\mathCodeExample{\geodesic<s>}
		\par\mathCodeExample{\geodesic<s>(t)} %chktex 36
		\par\mathCodeExample{\geodesic<l>{p}{q}}
		\par\mathCodeExample{\geodesic<l>{p}{q}(t)} %chktex 36
		\par\mathCodeExample{\geodesic<a>{p}{q}}
		\par\mathCodeExample{\geodesic<a>[Big]{p}{q}(\dfrac{t}{2})} %chktex 36
		\par\mathCodeExample{\geodesic<p>{p}{X}}
		\par\mathCodeExample{\geodesic<p>{p}{X}(t)} %chktex 36
		\par\mathCodeExample{\geodesic<p>[Big]{p}{X}(\dfrac{t}{2})} %chktex 36
		\par\mathCodeExample{\geodesic[big]{p}{X}((1-t)t)} %chktex 36
		\par\mathCodeExample{\geodesic|\dot\gamma|{p}{X}(t)} %chktex 36
	\item[geodesicSymbol] symbol to use for the geodesic in \codeCommand{\geodesic}
		\par\mathCodeExample{\geodesicSymbol}
	\item[inverseRetract] use an inverse retraction, the arguments are similar to \codeCommand{\logarithm} but use the \codeCommand{\retractionSymbol}
	\par\mathCodeExample{\inverseRetract{p}q}
	\par\mathCodeExample{\inverseRetract{p}(q)}
	\par\mathCodeExample{\inverseRetract[Big]{p}(q)}
	\item[logarithm] the logarithmic map.
		Its syntax is \codeCommand{\logarithm[#1]{#2}{#3}}.
		The first argument can be used to scale the third.
		The second argument denotes the base point.
		The third argument denotes another point, which is optional, but
		if provided, the argument is put in brackets. The first following example
		illustrates the case, where no brackets are put. Note that the space is
		mandatory.
		\par\mathCodeExample{\logarithm{p}q}
		\par\mathCodeExample{\logarithm{p}(q)}
		\par\mathCodeExample{\logarithm[Big]{p}(q)}
	\item[logOp] the symbol used within the \codeCommand{\logarithm}.
		\par\mathCodeExample{\logOp}
	\item[parallelTransport] the parallel transport.\\
		Its syntax is \codeCommand{\parallelTransport[#1]{#2}{#3}(#4){5}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument \#4.\cref{footnote:amsmath_sizes}
		The second argument is the start point of parallel transport on a manifold.
		The third argument is the end point of parallel transport on a manifold.
		The fourth (optional) argument is the tangent vector that is transported.
		Putting it in brackets enables the scaling by the first argument.
		The fifth (optional) argument specifies an exponent, for example to parallel transport along a curve $c$
		\par\mathCodeExample{\parallelTransport{p}{q}X}
		\par\mathCodeExample{\parallelTransport{p}{q}(X)}
		\par\mathCodeExample{\parallelTransport[big]{p}{q}(X)}
		\par\mathCodeExample{\parallelTransport{p}{q}(X)[c]}
		\par\mathCodeExample{\parallelTransport{p}{q}[c]}
	\item[parallelTransportDir] similar to \codeCommand{\parallelTransport}, but the third
		argument is a direction to transport into. This can be rewritten to the classical notation
		applying an exponential map from the base point (\#2) to th direction (\#3).
		The fifth (optional) argument specifies an exponent, for example to parallel transport along a curve $c$
		\par\mathCodeExample{\parallelTransportDir{p}{Y}X}
		\par\mathCodeExample{\parallelTransportDir{p}{Y}(X)}
		\par\mathCodeExample{\parallelTransportDir[big]{p}{Y}(X)}
		\par\mathCodeExample{\parallelTransportDir{p}{Y}(X)[c]}
		\par\mathCodeExample{\parallelTransportDir{p}{Y}[c]}
	\item[parallelTransportSymbol]\hspace{4em}the symbol to use within \codeCommand{\parallelTransport} and \codeCommand{\parallelTransportDir}
		\par\mathCodeExample{\parallelTransportSymbol}
	\item[retract] a retraction.\\
		Its syntax is \codeCommand{\retract[#1]{#2}{#3}}.
		The first argument can be used to scale the third.
		The second argument denotes the base point.
		The third argument denotes the tangent vector, which is optional, but
		if provided, the argument is put in brackets. The first following example
		illustrates the case, where no brackets are put. Note that the space is
		mandatory.
		\par\mathCodeExample{\retract{p}X}
		\par\mathCodeExample{\retract{p}(X)}
		\par\mathCodeExample{\retract[Big]{p}(\frac{X}{2})}
	\item[retractionSymbol] symbol to use for a retraction and an inverse retraction,
		see \codeCommand{\retract} and \codeCommand{\inverseRetract}.
		\par\mathCodeExample{\retractionSymbol}
	\item[riemannian] the Riemannian metric (family of inner products on the tangent spaces).
		Its syntax is \codeCommand{\riemannian[#1]{#2}{#3}[#4]}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the first factor.
		The third argument denotes the second factor.
		The fourth (optional) argument denotes the base point of the tangent space.
		\par\mathCodeExample{\riemannian{X_1}{X_2}}
		\par\mathCodeExample{\riemannian{Y_1}{Y_2}[q]}
		\par\mathCodeExample{\riemannian[Big]{\dfrac{1}{2}X_1}{X_2}[p]}
	\item[riemanniannorm] the norm induced by the Riemannian metric.
		Its syntax is \codeCommand{\riemanniannorm[#1]{#2}[#3]}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the argument.
		The third (optional) argument denotes the base point of the tangent space.
		\par\mathCodeExample{\riemanniannorm{X}}
		\par\mathCodeExample{\riemanniannorm{Y}[p]}
		\par\mathCodeExample{\riemanniannorm[Big]{\dfrac{1}{2}X}[p]}
	\item[secondCovariantDerivative]\hspace{4em}is the second-order covariant derivative.
		Its syntax is \codeCommand{\secondCovariantDerivative{#1}{#2}[#3]}.
		The first argument is the vector (or vector field) determining the first direction of differentiation.
		The second argument is the vector (or vector field) determining the second direction of differentiation.
		The third (optional) argument denotes the tensor field being differentiated.
		\par\mathCodeExample{\secondCovariantDerivative{X}{Y}{T}}
	\item[secondCovariantDerivativeSymbol]\hspace{4em}the symbol used for the second covariant derivative \codeCommand{\secondCovariantDerivative}.
		\par\mathCodeExample{\secondCovariantDerivativeSymbol}
	\item[tangent] the tangent space.
		Its syntax is \codeCommand{\tangent{#1}[#2]}.
		The first argument denotes the base point.
		The second (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\tangent{p}}
		\par\mathCodeExample{\tangent{q}[\cN]}
	\item[tangentBundle] the tangent bundle.
		Its syntax is \codeCommand{\tangentBundle[#1]}.
		The (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\tangentBundle}
		\par\mathCodeExample{\tangentBundle[\cN]}
	\item[tangentSpaceSymbol] the symbol used within \codeCommand{\tangent}.
		\par\mathCodeExample{\tangentSpaceSymbol}
	\item[tensorBundle] the tensor bundle.
		Its syntax is \codeCommand{\tensorBundle{#1}{#2}[#3]}.
		The first argument denotes the number $r$ of elements of the cotangent space the tensors accept.
		The second argument denotes the number $s$ of elements of the tangent space the tensors accept.
		The third (optional) argument denotes the manifold, which defaults to $\cM$.
		\par\mathCodeExample{\tensorBundle{r}{s}}
		\par\mathCodeExample{\tensorBundle{r}{s}[\cN]}
	\item[tensorSpace] a tensor space over a vector space~$V$.
		Its syntax is \codeCommand{\tensorSpace{#1}{#2}[#3]}.
		The first argument denotes the number $r$ of elements of the dual space~$V^*$ the tensors accept.
		The second argument denotes the number $s$ of elements of the space~$V$ the tensors accept.
		The third (optional) argument denotes the vector space, which defaults to empty.
		\par\mathCodeExample{\tensorSpace{r}{s}}
		\par\mathCodeExample{\tensorSpace{r}{s}[V]}
	\item[tensorSpaceSymbol] the symbol used within \codeCommand{\tensorSpace} and \codeCommand{\tensorBundle}.
		\par\mathCodeExample{\tensorSpaceSymbol}
	\item[vectorTransport] a vector transport.\\
		Its syntax is \codeCommand{\vectorTransport[#1]{#2}{#3}(#4)[#5]}.
		The first (optional) argument is used to scale the parantheses enclosing the argument \#4.\cref{footnote:amsmath_sizes}
		The second argument is the start point of vector transport on a manifold.
		The third argument is the end point of vector transport on a manifold.
		The fourth (optional) argument is the tangent vector that is transported.
		Putting it in brackets enables the scaling by the first argument.
		Finally a retraction symbol can be added in the exponent to distinguish vector transports as \#5.
		\par\mathCodeExample{\vectorTransport{p}{q}X}
		\par\mathCodeExample{\vectorTransport{p}{q}(X)}
		\par\mathCodeExample{\vectorTransport[big]{p}{q}(X)}
		\par\mathCodeExample{\vectorTransport{p}{q}(X)[\retractionSymbol]}
	\item[vectorTransportDir] similar to \codeCommand{\vectorTransport}, but the third
		argument is a direction to transport into. This can be rewritten to the classical notation
		applying an retraction from the base point (\#2) to th direction (\#3).
		\par\mathCodeExample{\vectorTransportDir{p}{Y}X}
		\par\mathCodeExample{\vectorTransportDir{p}{Y}(X)}
		\par\mathCodeExample{\vectorTransportDir[big]{p}{Y}(X)}
		\par\mathCodeExample{\vectorTransportDir{p}{Y}(X)[\retractionSymbol]}
	\item[vectorTransportSymbol]\hspace{4em}the symbol to use within \codeCommand{\vectorTransport} and \codeCommand{\vectorTransportDir}
		\par\mathCodeExample{\vectorTransportSymbol}
\end{commandlist}


\subsection{Optimization: \texorpdfstring{\file{numapde-optimization.sty}}{numapde-optimization.sty}}\label{subsec:optimization}

The semantic file \file{numapde-optimization.sty} collects definitions and notations related to optimization.
\begin{commandlist}
	\item[linearizingcone] the linearizing cone.
		Its syntax is \codeCommand{\linearizingcone[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the base point.
		\par\mathCodeExample{\linearizingcone{A}{x}}
		\par\mathCodeExample{\linearizingcone{A}{x^2}}
		\par\mathCodeExample{\linearizingcone[big]{A}{x^2}}

	\item[normalcone] the normal cone.
		Its syntax is \codeCommand{\normalcone[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the base point.
		\par\mathCodeExample{\normalcone{A}{x}}
		\par\mathCodeExample{\normalcone{A}{x^2}}
		\par\mathCodeExample{\normalcone[big]{A}{x^2}}

	\item[polarcone] the polar cone of a set \mathCodeExample{\polarcone{A}}

	\item[radialcone] the radial cone.
		Its syntax is \codeCommand{\radialcone[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the base point.
		\par\mathCodeExample{\radialcone{A}{x}}
		\par\mathCodeExample{\radialcone{A}{x^2}}
		\par\mathCodeExample{\radialcone[big]{A}{x^2}}

	\item[tangentcone] the tangent cone.
		Its syntax is \codeCommand{\tangentcone[#1]{#2}{#3}}.
		The first (optional) argument is used to scale the parantheses enclosing the argument to the standard amsmath sizes.\cref{footnote:amsmath_sizes}
		The second argument denotes the set.
		The third argument denotes the base point.
		\par\mathCodeExample{\tangentcone{A}{x}}
		\par\mathCodeExample{\tangentcone{A}{x^2}}
		\par\mathCodeExample{\tangentcone[big]{A}{x^2}}
\end{commandlist}

\section{Translations: \texorpdfstring{\file{numapde-translations.sty}}{numapde-translations.sty}}\label{sec:translation}
This currently optional addition loads \lstinline!translations.sty! to define translations as well as \lstinline!babel.sty! to set the language properly. 
Currently only a German dictionary is provided while the default fallback (or name of the keys) is English, see \lstinline!numapde-german.trsl!. 
The list currently covers

\begin{dictionarylist}
\PrintDictionaryFor{German}{numapde}{\item[}{]}{}
\end{dictionarylist}

\section{Document Classes}\label{sec:documentclasses}
There are several document classes within this package, providing help with preprint, skripts, exercise sheets and theses.
Since all follow a common style, the file \lstinline!numapde-cls-commons.sty!. This file \emph{first} loads the syntax, see \cref{sec:syntax},
then the following packages are loaded and only \emph{after that} the semantics are loaded, see \cref{sec:semantic} as well as the dictionary from \cref{sec:translation}.

\paragraph{Packages.}
\begin{commandlist}
	\item[\file{libertine.sty}] for the text font
	\item[\file{lastpage.sty}] for configuring the footer (and display the last page's number)
	\item[\file{microtype.sty}] for micro-typographic extensions
	\item[\file{newtxmath.sty}] for the math font
	\item[\file{inconsolata.sty}] for the numbers font
	\item[\file{scrdate.sty}] for getting a formated date
	\item[\file{scrlayer-scrpage.sty}] for the page layout
\end{commandlist}

\paragraph{Commands.} The following commands can be used in headers or in making a title page.
internally these values stored within a \lstinline!numapde@! variable, e.g. for the \lstinline!\shorttitle! sets \lstinline!\numapde@shorttitle!.
\begin{commandlist}
    \item[shortauthor] set a short author(s) string for the headers
    \item[shorttitle] set a short title string for the headers
    \item[acknowledgements] set acknowledgements
    \item[acknowledgments] set acknowledgements, an alias of the previous command
    \item[manuscriptlicense] set a license, This is by default set to \codeExample{\ccbyncsa}
    \item[manuscriptcopyright] set a copyright note
\end{commandlist}

\subsection{\texorpdfstring{\file{numapde-preprint.cls}}{numapde-preprint.cls}}
The documentclass \file{numapde-preprint.cls} can be used to typeset preprints. It is based on \file{scrartcl.cls}.
It additionally uses the folloing packages. These are loaded \emph{after} the aforementioned semantics, but \emph{before} adding the style and colors.
% Last updated: 04.10.2019 from numapde-preprint.cls

\paragraph{Options.}
\begin{commandlist}
	\item[lineno] can be used to activate line numbers
\end{commandlist}
all other document options are passed on to \lstinline!scrartcl!.

\paragraph{Packages.}
\begin{commandlist}
	\item[\file{lineno.sty}] for line numbers
	\item[\file{truncate.sty}] to shorten texts on headers and footers
\end{commandlist}

\paragraph{Environments.}
\begin{commandlist}
	\item[keywords] to specify keywords used at the beginning of the preprint
	\item[AMS] to specify the AMS classificatiobs of the preprint
\end{commandlist}

\subsection{\texorpdfstring{\file{numapde-thesis.cls}}{numapde-thesis.cls}}
The documentclass \file{numapde-thesis.cls} can be used to typeset theses. It is based on \file{scrreprt.cls}.
It additionally uses the following packages. These are loaded \emph{after} the aforementioned semantics, but \emph{before} adding the style and colors.
% Last updated: 24.04.2020 from numapde-thesis.cls

\paragraph{Options.}
\begin{commandlist}
	\item[lineno] can be used to activate line numbers
\end{commandlist}
all other document options are passed on to \lstinline!scrreprt!.

\paragraph{Packages.}
\begin{commandlist}
	\item[\file{lineno.sty}] for line numbers
	\item[\file{pdfpages.sty}] to include the declaration of authorship
\end{commandlist}

\paragraph{Commands.} The following commands are mainly used to set values on the title page and the headers.
\begin{commandlist}
	\item[thesis] to set the type of thesis, for example \lstinline!\GetTranslation{bachelor thesis}! to get the localized version of a bachelor thesis set.
	\item[degree] to set the type of degree the thesis is for
	\item[studentID] for the student number
	\item[submissiondate] to set the date of submission
	\item[firstsupervisor] to set the first supervisor
	\item[secondsupervisor] to set the second supervisor
	\item[supervisornote] add a note below the supervisors, for example to mention that the thesis was supervised by a company.
	\item[logo] to set the logo being included with \lstinline!\includegraphics!. This is by default set to \lstinline!logo/TU_Chemnitz_Logo_gruen_RGB.png!, i.e. you need the logo from the university in that folder for this to work properly. This is not included (for legal reasons) within this repository.
\end{commandlist}
The title page is automatically localized to the language chosen using the translations from \cref{sec:translation}

\subsection{\texorpdfstring{\file{numapde-teaching.sty}}{numapde-teaching.sty}}\label{sec:teaching}
This class collects common commands and environments for teaching classes that follow in the next subsections. This of course first loads \file{numapde-cls-commons.sty}.

\paragraph{Options.}
\begin{commandlist}
	\item[final] activates \lstinline!noextras! and \lstinline!nosolutions!
	\item[noextras] disable printing of extra information as well as \lstinline!todonotes!
	\item[nosolutions] disable printing of solutions
\end{commandlist}

\paragraph{Commands.}
\begin{commandlist}
	\item[alert] similar to \lstinline!alert! in beamer it defines alerted text
	\item[courseurl] url to the course's homepage
	\item[EndOfClass] add a marker to indicate an end of a class
	\item[EndOfWeek] add a marker to indicate an end of a week
	\item[lecture] name of the lecture
	\item[numapdeQuestion] to formulate a question (for students to read or to ask in class)
	\item[numapdeNote] to formulate a question (for students to read or to ask in class)
	\item[numapdeAnswer] so answe a \lstinline!numapdeQuestion!. Thes only show up without \lstinline!noextra! activated
	\item[team] the team accompanying the lecture.
\end{commandlist}

\paragraph{Environments.}
\begin{commandlist}
	\item[numapdeExtra] an environmant only set if \lstinline!noextra! is not set, i.e. the script contains extra info
	\item[numapdeProblem] formulate a problem, for example also in the exercise
	\item[numapdeSolution] the solution to a problem, only shows up if \lstinline!nosolution! is not set
\end{commandlist}
\subsection{\texorpdfstring{\file{numapde-lecture-notes.cls}}{numapde-lecture-notes.cls}}
This class is a \lstinline!scrreprt! class based on \lstinline!numapde-teaching.sty! from \cref{sec:teaching}.
\subsection{\texorpdfstring{\file{numapde-exercise.cls}}{numapde-exercise.cls}}
This class is a \lstinline!scrartcl! class based on \lstinline!numapde-teaching.sty! from \cref{sec:teaching}.


\section{Colors: \texorpdfstring{\file{numapde-colors.sty}}{numapde-colors.sty}}\label{sec:colors}

The colors defined in \file{numapde-colors.sty} are a collection mainly of Paul Tol's notes on colors.\footnote{see \url{https://personal.sron.nl/~pault/}}
Currently the schemes
\begin{itemize}
	\item high contrast
		\par\colorExample{TolHighContrastWhite}
		\par\colorExample{TolHighContrastYellow}
		\par\colorExample{TolHighContrastRed}
		\par\colorExample{TolHighContrastBlue}
		\par\colorExample{TolHighContrastBlack}
	\item bright
		\par\colorExample{TolBrightBlue}
		\par\colorExample{TolBrightCyan}
		\par\colorExample{TolBrightGreen}
		\par\colorExample{TolBrightYellow}
		\par\colorExample{TolBrightRed}
		\par\colorExample{TolBrightPurple}
		\par\colorExample{TolBrightGray}
	\item vibrant
		\par\colorExample{TolVibrantBlue}
		\par\colorExample{TolVibrantCyan}
		\par\colorExample{TolVibrantTeal}
		\par\colorExample{TolVibrantOrange}
		\par\colorExample{TolVibrantRed}
		\par\colorExample{TolVibrantMagenta}
		\par\colorExample{TolVibrantGray}
	\item muted
		\par\colorExample{TolMutedBlue}
		\par\colorExample{TolMutedCyan}
		\par\colorExample{TolMutedTeal}
		\par\colorExample{TolMutedGreen}
		\par\colorExample{TolMutedOlive}
		\par\colorExample{TolMutedSand}
		\par\colorExample{TolMutedRose}
		\par\colorExample{TolMutedWine}
		\par\colorExample{TolMutedPurple}
	\item pale
		\par\colorExample{TolPaleBlue}
		\par\colorExample{TolPaleCyan}
		\par\colorExample{TolPaleGreen}
		\par\colorExample{TolPaleYellow}
		\par\colorExample{TolPaleRed}
		\par\colorExample{TolPaleGray}
	\item dark
		\par\colorExample{TolDarkBlue}
		\par\colorExample{TolDarkCyan}
		\par\colorExample{TolDarkGreen}
		\par\colorExample{TolDarkYellow}
		\par\colorExample{TolDarkRed}
		\par\colorExample{TolDarkGray}
	\item light
		\par\colorExample{TolLightBlue}
		\par\colorExample{TolLightCyan}
		\par\colorExample{TolLightMint}
		\par\colorExample{TolLightPear}
		\par\colorExample{TolLightOlive}
		\par\colorExample{TolLightYellow}
		\par\colorExample{TolLightOrange}
		\par\colorExample{TolLightPink}
\end{itemize}
are transcribed from Paul Tol's notes.


\section{Style: \texorpdfstring{\file{numapde-style.sty}}{numapde-style.sty}}\label{sec:style}

The style file \file{numapde-style.sty} is used to define a unified style by configuration of a number of packages loaded in \file{numapde-packages.sty}.
The following packages are currently being configured here:
% Last updated: 03.11.2020 from numapde-style.sty

\begin{description}
	\item[\file{biblatex.sty}]
	\item[\file{changes.sty}]
	\item[\file{chngcntr.sty}]
	\item[\file{cleveref.sty}]
	\item[\file{enumitem.sty}]
	\item[\file{hyperref.sty}]
	\item[\file{listings.sty}]
	\item[\file{url.sty}]
\end{description}


\section{How to use \texorpdfstring{\file{numapde-local.sty}}{numapde-local.sty}}\label{sec:local-definitions}

To keep the main document free from clutter, all packages to be loaded in addition to those in \file{numapde-packages.sty} should be \codeCommand{\RequirePackage}:d in here.
Moreover, additional commands not found in any of the other \file{numapde-*.sty} files go in here.

If you feel like a command or package is useful for multiple documents and should be included by default, please consult the authors of this document.


\paragraph{Example.}

For this document, a number of commands were introduced locally in \file{numapde-local.sty}, including \codeCommand{\mathCodeExample}, which displays a \LaTeX{} code snippet and renders it as inline math.

\end{document}

